Pointwise-Sparse Actuator Scheduling for Linear Systems with Controllability Guarantee

This paper considers the design of sparse actuator schedules for linear time-invariant systems. An actuator schedule selects, for each time instant, which control inputs act on the system in that instant. We address the optimal scheduling of control inputs under a hard constraint on the number of inputs that can be used at each time. For a sparsely controllable system, we characterize sparse actuator schedules that make the system controllable, and then devise a greedy selection algorithm that guarantees controllability while heuristically providing low control effort. We further show how to enhance our greedy algorithm via Markov chain Monte Carlo-based randomized optimization

==> Sections/Proof_Theorem1.tex <==
%!TEX root = ../LCSS-sparse_control.tex

\subsection{Proof of \Cref{lem:suff}}\label{app:suff}

We define the matrix $\bs{K}^{(k)}=\bs{I}-\bs{A}^k(\bs{A}^k)^{\dagger}$,
where $(\cdot)^{\dagger}$ denotes the pseudoinverse of a matrix, as the projection matrix onto $\keril{(\bs{A}^{k})^\top}$. 
As the subspace orthogonal to $\keril{(\bs{A}^{k})^\top}$ is $\imil{\bs{A}^{k}}$, we get
\begin{equation}\label{eq:orthogonalspaces}
	\ker{\lb\bs{A}^{k}\rb^\top} \ominus \ker{\lb\bs{A}^{k-1}\rb^\top} = \im{\bs{K}^{(k)}\bs{A}^{k-1}}.
\end{equation}
We note that~\eqref{eq:suff_feasibility} trivially holds if $R=0$ by setting $k=R+1$.
Then,
from~\eqref{eq:orthogonalspaces},
to prove~\eqref{eq:suff_feasibility} for all $k\in[R]$ it suffices to prove that there exists an index set $\cl{S}_{h-k}$ for each $k\in[R]$ such that
\begin{equation}\label{eq:suff_condition}
	\im{\bs{K}^{(k)}\bs{A}^{k-1}} = \im{\bs{K}^{(k)}\bs{A}^{k-1}\bs{B}_{\cl{S}_{h-k}}}. 
\end{equation}
Since the system is controllable,
it holds
\begin{equation} \label{eq:span_AB}
	\begin{aligned}
		\im{\bs{K}^{(k)}\bs{A}^{k-1}} &=\im{\bs{K}^{(k)}\bs{A}^{k-1}\bs{\Phi}^n} \\
		&=\im{\bs{K}^{(k)}\bs{A}^{k-1}\bs{B}},
	\end{aligned}
\end{equation}
because $\bs{K}^{(k)}\bs{A}^{k-1}\bs{A}^i=[\bs{I}-\bs{A}^{k}(\bs{A}^{k})^{\dagger}]\bs{A}^{k}\bs{A}^{i-1}=\bs{0}$, for $i>0$. 
Applying the Sylvester rank inequality to~\eqref{eq:orthogonalspaces} yields 
\begin{multline}
	\rank{\bs{K}^{(k)}\bs{A}^{k-1}} =\ls n-\rank{\bs{A}^{k}} \rs-\ls n-\rank{\bs{A}^{k-1}}\rs\\
	=\rank{\bs{A}^{k-1}} - \rank{\bs{A}^{k}}    \leq n-\rank{\bs{A}}\leq s.
\end{multline}
From \eqref{eq:span_AB}, we conclude that there exist $s$ columns in $\bs{K}^{(k)}\bs{A}^{k-1}\bs{B}$,
indexed by $\cl{S}_{h-k}$,
such that \eqref{eq:suff_condition} holds.
Also, for any $\bs{z}\in\keril{(\bs{A}^R)^{\top}}$, we have $\bs{z} = [\bs{I}-\bs{K}^{(1)}]\bs{z}+\bs{K}^{(1)}\bs{z}$. Here, $\bs{K}^{(1)}\bs{z}=\bs{K}^{(1)}\bs{B}_{\sch[h-1]}\bs{v}(h-1)$
for some $\bs{v}(h-1)$ due to \eqref{eq:suff_condition} with $k=1$. 
Hence, defining $\bar{\bs{z}}(1) \doteq  [\bs{I}-\bs{K}^{(1)}][\bs{z}-\bs{B}_{\sch[h-1]}\bs{v}(h-1)]$, we have
\begin{equation}
	\bs{z} = \bar{\bs{z}}(1)+\bs{B}_{\sch[h-1]}\bs{v}(h-1).
\end{equation}
Recursively using \eqref{eq:suff_condition}, there exist $\{\bs{v}(k)\}_{k=1}^R$ such that
\begin{equation}\label{eq:z}
	\begin{aligned}
		\bs{z} &= \ls \bs{I}-\bs{K}^{(2)}\rs\bar{\bs{z}}(1)+\bs{K}^{(2)}\bar{\bs{z}}(1)+\bs{B}_{\sch[h-1]}\!\bs{v}(h-1)\\
		&= \bar{\bs{z}}(2)+\sum_{k=1}^{2}\bs{A}^{k-1}\bs{B}_{\sch[h-k]}\bs{v}(h-2)\\
		&=\bar{\bs{z}}(R)+\sum_{k=1}^{R}\bs{A}^{k-1}\bs{B}_{\sch[h-k]}\bs{v}(h-k),
	\end{aligned}
\end{equation}
where $\bar{\bs{z}}(k)=\ls \bs{I}-\bs{K}^{(k)}\rs\ls \bar{\bs{z}}(k-1)-\bs{B}_{\sch[h-k]}\bs{v}(h-k)\rs$.
Since $\bs{z}\in\keril{(\bs{A}^R)^{\top}}$, multiplying~\eqref{eq:z} with $\bs{K}^{(R)}$ gives 
\begin{equation}
	\bs{K}^{(R)}\bs{z}=\bs{z} = \bs{K}^{(R)}\sum_{k=1}^{R}\bs{A}^{k-1}\bs{B}_{\sch[h-k-1]}\bs{v}(k),
\end{equation}
proving the desired result \eqref{eq:span_null}.
